Enhancing Fiber Orientation Distributions using convolutional Neural Networks

Accurate local fiber orientation distribution (FOD) modeling based on diffusion magnetic resonance imaging (dMRI) capable of resolving complex fiber configurations benefits from specific acquisition protocols that sample a high number of gradient directions (b-vecs), a high maximum b-value(b-vals), and multiple b-values (multi-shell). However, acquisition time is limited in a clinical setting and commercial scanners may not provide such dMRI sequences. Therefore, dMRI is often acquired as single-shell (single b-value). In this work, we learn improved FODs for commercially acquired MRI. We evaluate patch-based 3D convolutional neural networks (CNNs)on their ability to regress multi-shell FOD representations from single-shell representations, where the representation is a spherical harmonics obtained from constrained spherical deconvolution (CSD) to model FODs. We evaluate U-Net and HighResNet 3D CNN architectures on data from the Human Connectome Project and an in-house dataset. We evaluate how well each CNN model can resolve local fiber orientation 1) when training and testing on datasets with the same dMRI acquisition protocol; 2) when testing on a dataset with a different dMRI acquisition protocol than used to train the CNN models; and 3) when testing on a dataset with a fewer number of gradient directions than used to train the CNN models. Our approach may enable robust CSD model estimation on single-shell dMRI acquisition protocols with few gradient directions, reducing acquisition times, facilitating translation of improved FOD estimation to time-limited clinical environments.

==> files/cdf_exp3.tex <==
\begin{figure*}[!htb]
\begin{center}
\includegraphics[width=\textwidth]{figs/acc_cdf_exp_3.eps}
\end{center}
\caption{\label{fig:acc_cdf_exp3} ACC Cumulative distribution functions (CDFs) for Experiment 3. The ideal ACC would give a single peak at one. HR = HighResNet.}
\end{figure*}

==> files/table_exp3.tex <==
\begin{table*}[!htb]
\centering
\caption{\label{tab:acc_exp_3} MAE and ACC mean, std and median between M-CSD and CSD model coefficients for Experiment 3. The minimum MAE and maximum ACC mean and median are in bold. The label \textit{Train} indicates data used to train the \textit{CNNs} and the \textit{Test} indicates the dataset used for the inference. HR = HighResNet.}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{\textbf{Train-Test}} 
& \multirow{2}{*}{\textbf{Method}}
& \textbf{MAE} 
& \multicolumn{2}{c}{\textbf{ACC}} 
\\\cmidrule{3-5}
&
& mean(std) 
& mean(std) 
& median 
\\\midrule
- & \textit{2TS-CSD} (QS 700) & 1.076(0.088) & 0.819(0.144) & 0.846\\\cdashline{2-5}
\multirow{2}*{QS 700-QS 700} 
& \textit{CNN}  HR & 0.529(0.052) & 0.901(0.112) & 0.939 \\
& \textit{CNN}  U-Net & \textbf{0.521(0.045)} & \textbf{0.902(0.116)} & \textbf{0.941}\\\cdashline{2-5}
\multirow{2}*{HCP 2000-QS 700}
& \textit{CNN}  HR & 0.771(0.075) & 0.882(0.117) & 0.921\\
& \textit{CNN}  U-Net & 0.777(0.069) & 0.877(0.114) & 0.911\\
\midrule
- & \textit{2TS-CSD} (QS 2500) & 0.964(0.077) & 0.888(0.12) & 0.930\\\cdashline{2-5}
\multirow{2}*{QS 2500-QS 2500}
& \textit{CNN}  HR & \textbf{0.411(0.04)} & \textbf{0.930(0.096)} & \textbf{0.964}\\
& \textit{CNN}  U-Net & 0.421(0.039) & 0.928(0.098) & 0.962\\\cdashline{2-5}
\multirow{2}*{HCP 2000-QS 2500}
& \textit{CNN}  HR & 0.493(0.047) & 0.924(0.094) & 0.957\\
& \textit{CNN}  U-Net & 0.536(0.039) & 0.922(0.094) & 0.955\\
\midrule
- & \textit{2TS-CSD} (HCP 2000) & 0.852(0.141) & 0.889(0.117) & 0.929\\\cdashline{2-5}
 \multirow{2}*{HCP 2000-QS 2000} 
& \textit{CNN}  HR & 0.338(0.052) & \textbf{0.948(0.077)} & \textbf{0.977} \\
& \textit{CNN}  U-Net & \textbf{0.337(0.051)} & \textbf{0.948(0.077)} & \textbf{0.977}\\\cdashline{2-5}
\multirow{2}*{QS 700-HCP 2000}
& \textit{CNN}  HR & 0.588(0.082) & 0.933(0.079) & 0.964 \\
& \textit{CNN}  U-Net & 0.677(0.081) & 0.936(0.082) & 0.966 \\\cdashline{2-5}
\multirow{2}*{QS 2500-HCP 2000}
& \textit{CNN}  HR & 0.510(0.093) & 0.927(0.088) & 0.960 \\
& \textit{CNN}  U-Net & 0.509(0.100) & 0.924(0.099) & 0.960 \\
\bottomrule
\end{tabular}
}
\end{table*}

















